Decentralization and Acceleration Enables Large-Scale Bundle Adjustment

Scaling to arbitrarily large bundle adjustment problems requires data and compute to be distributed across multiple devices. Centralized methods in prior works are only able to solve small or medium size problems due to overhead in computation and communication. In this paper, we present a fully decentralized method that alleviates computation and communication bottlenecks to solve arbitrarily large bundle adjustment problems. We achieve this by reformulating the reprojection error and deriving a novel surrogate function that decouples optimization variables from different devices. This function makes it possible to use majorization minimization techniques and reduces bundle adjustment to independent optimization subproblems that can be solved in parallel. We further apply Nesterov's acceleration and adaptive restart to improve convergence while maintaining its theoretical guarantees. Despite limited peer-to-peer communication, our method has provable convergence to first-order critical points under mild conditions. On extensive benchmarks with public datasets, our method converges much faster than decentralized baselines with similar memory usage and communication load. Compared to centralized baselines using a single device, our method, while being decentralized, yields more accurate solutions with significant speedups of up to 953.7x over Ceres and 174.6x over DeepLM. Code: https://joeaortiz.github.io/daba.

==> algorithms/algorithm_mm.tex <==
\begin{algorithm}[t]
	\caption{The $\mm$ Method}
	\label{algorithm::mm}
	\begin{algorithmic}[1]
		\State\textbf{Input}: An initial iterate $\bfx^{(0)}\in $ and $\xi > 0$.
		\State\textbf{Output}: A sequence of iterates $\{\bfxk\}$.\vspace{0.2em} 
		\For{$\sfk\gets 0,\,1,\,2,\,\cdots$}
		\For{ each device $\alpha\in\calS$}
        \State{\color{gray} // Inter-device communication}
		\State 	retrieve $\bfxbk$ from neighboring devices $\beta$
        \State{\color{gray} // Majorization}
		\State  construct $\Ealphak$ with \cref{eq::Ealpha}
        \State{\color{gray} // Minimization}
		\State  solve $\bfxakp\leftarrow\arg\min_{\bfxa} \Ealphak$
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}


==> table/table_cmp_datasets_huber.tex <==
\begin{table*}[t]
    \renewcommand{\arraystretch}{1.15}
	\setlength{\tabcolsep}{0.625em}
	\centering
	\caption{Mean reprojection errors using the \textbf{\color{blue}Huber loss} for decentralized methods $\dr$ \cite{eriksson2016consensus}, $\admm$ \cite{zhang2017dist}, $\amm$ (ours) with \textbf{4, 8, 16, 32 devices} on the datasets in \cref{table::dataset}. Each decentralized method is run with 1000 iterations. The results from centralized methods $\ceres$ \cite{ceres-solver}  with 40 iterations are used as references. For each setup, a decentralized  method is  marked in \textbf{bold} if achieving the best result and colored in {\color{red} red} if outperforming $\ceres$ and $\deeplm$. Note that $\deeplm$ \cite{huang2021deeplm} does not support the Huber or other robust losses.} \label{table::comp_huber}
	\begin{tabular}{|c|c|c||c|c|c||c|c|c||c|c|c||c|c|c|}
		% \hline
  %       \multicolumn{16}{|c|}{\multirow{2}{*}{Huber Loss}}\\
  %       \multicolumn{16}{|c|}{}\\
        \hline
		\multirow{3}{*}{Dataset}& \multicolumn{14}{c|}{Mean Reprojection Error}\\
		\cline{2-15}
		& \multirow{2}{*}{Init} & \multirow{2}{*}{$\ceres$}  &  \multicolumn{3}{c||}{4 Devices} & \multicolumn{3}{c||}{8 Devices} & \multicolumn{3}{c||}{16 Devices} & \multicolumn{3}{c|}{32 Devices}\\
		\cline{4-15}
		& & &  {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$}  & {\scriptsize $\amm$}  & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} &  {\scriptsize $\amm$}\\
		\hline
  		\hline
		\multicolumn{15}{|c|}{BAL \cite{agarwal2010bundle}}\\
        \hline
        {\scriptsize\sf Ladybug} & {3.267} & {0.703}  &{0.838} & {\color{red}0.693} & \textbf{\color{red}0.690} & {0.839} & {\color{red}0.694} & \textbf{\color{red}0.690} & {0.842} & {\color{red}0.694} & \textbf{\color{red}0.690} & {0.844} & {\color{red}0.694} & \textbf{\color{red}0.690} \\
        \hline
        {\scriptsize\sf Venice} & {4.750} & {0.467}  &{0.515} & {0.534} & \textbf{\color{red}0.465} & {0.515} & {0.541} & \textbf{\color{red}0.465} & {0.517} & {0.651} & \textbf{\color{red}0.467} & {0.518} & {0.727} & \textbf{0.473} \\
        \hline
        {\scriptsize\sf Final} & {7.573} & {0.820}  &{2.009} & {0.910} & \textbf{\color{red}0.808} & {2.064} & {0.945} & \textbf{\color{red}0.810} & {2.099} & {0.957} & \textbf{\color{red}0.812} & {2.205} & {0.961} & \textbf{0.826} \\
        \hline
        \hline
        \multicolumn{15}{|c|}{1DSfM \cite{wilson2014robust}}\\
		\hline
        {\scriptsize\sf Gen. Markt} & {8.031} & {3.943}  &{4.790} & {4.293} & \textbf{\color{red}3.928} & {4.810} & {4.383} & \textbf{\color{red}3.938} & {4.855} & {4.489} & \textbf{3.951} & {4.892} & {4.651} & \textbf{3.972} \\
        \hline
        {\scriptsize\sf Piccadily} & {10.34} & {4.139}  &{5.780} & {4.210} & \textbf{\color{red}4.020} & {5.773} & {4.265} & \textbf{\color{red}3.943} & {5.855} & {4.360} & \textbf{\color{red}4.062} & {5.908} & {4.408} & \textbf{\color{red}4.049} \\
        \hline
        {\scriptsize\sf R. Forum} & {6.247} & {1.172}  &{2.146} & {1.473} & \textbf{\color{red}1.128} & {2.171} & {1.553} & \textbf{\color{red}1.153} & {2.206} & {1.648} & \textbf{1.186} & {2.219} & {1.732} & \textbf{1.191} \\
        \hline
        {\scriptsize\sf Trafalgar} & {9.901} & {3.492}  &{4.918} & {3.674} & \textbf{\color{red}3.402} & {4.893} & {3.768} & \textbf{\color{red}3.395} & {5.026} & {3.880} & \textbf{\color{red}3.449} & {5.060} & {4.024} & \textbf{\color{red}3.473} \\
        \hline
        {\scriptsize\sf U. Square} & {10.18} & {3.918}  &{5.253} & {4.056} & \textbf{\color{red}3.814} & {5.317} & {4.079} & \textbf{\color{red}3.810} & {5.373} & {4.166} & \textbf{\color{red}3.842} & {5.425} & {4.248} & \textbf{\color{red}3.882} \\
        \hline
        {\scriptsize\sf V. Cathedral} & {9.085} & {1.778}  &{3.027} & {1.982} & \textbf{\color{red}1.673} & {3.038} & {2.016} & \textbf{\color{red}1.664} & {3.099} & {2.108} & \textbf{\color{red}1.723} & {3.173} & {2.200} & \textbf{\color{red}1.730} \\
        \hline
	\end{tabular}
	\vspace{-0.75em}
\end{table*}

==> table/table_cmp_datasets_trivial_full.tex <==

\begin{table*}[p]
	\vspace{-1em}
	\renewcommand{\arraystretch}{1}
	\setlength{\tabcolsep}{0.31em}
	\centering
	\caption{Mean reprojection errors using the \textbf{\color{blue}trivial loss} for  $\mm$, $\amm$, $\dr$, $\admm$ on the datasets in \cref{table::dataset}. There are \textbf{4, 8, 16, 32 agents}.   \textbf{Init}: initial errors for all the methods.  \textbf{Ref}: reference errors from $\ceres$ \cite{ceres-solver} and $\deeplm$ \cite{huang2021deeplm}. \textbf{Iter}: errors of decentralized methods with \textbf{100, 500, 1000 iterations}. For each setup, a decentralized  method is  marked in \textbf{bold} if achieving the best performance and colored in {\color{red} red} if outperforming $\ceres$ \cite{ceres-solver} and $\deeplm$ \cite{huang2021deeplm}.} \label{table::comp_trivial}
	\begin{tabular}{|c|c|c|c|c|c|c|c||c|c|c|c||c|c|c|c||c|c|c|c|}
		\hline
		\multirow{3}{*}{Dataset}& \multicolumn{19}{c|}{Mean Reprojection Error}\\
		\cline{2-20}
		& \multirow{2}{*}{Init} & \multirow{2}{*}{Ref} & \multirow{2}{*}{Iter} & \multicolumn{4}{c||}{4 Devices} & \multicolumn{4}{c||}{8 Devices} & \multicolumn{4}{c||}{16 Devices} & \multicolumn{4}{c|}{32 Devices}\\
		\cline{5-20}
		& & & & {\scriptsize $\mm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} & {\scriptsize $\mm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} & {\scriptsize $\mm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} & {\scriptsize $\mm$} & {\scriptsize $\amm$} & {\,\scriptsize $\dr$\,} & {\scriptsize $\admm$} \\
		\cline{5-20}
		\hline
		\hline
		\multicolumn{20}{|c|}{BAL \cite{agarwal2010bundle}}\\
		\hline
		\multirow{3}{*}{\scriptsize\sf Trafalgar} & \multirow{3}{*}{1.527} & \multirow{3}{*}{0.453} & 100 & {0.511} & \textbf{0.478} & {1.187} & {1.527} & {0.519} & \textbf{0.486} & {1.144} & {1.527} & {0.529} & \textbf{0.489} & {1.246} & {1.527} & {0.537} & \textbf{0.494} & {1.144} & {0.960} \\
		\cline{4-20}
		& & & 500 & {0.487} & \textbf{0.462} & {0.494} & {0.477} & {0.498} & \textbf{0.464} & {0.495} & {0.483} & {0.503} & \textbf{0.467} & {0.496} & {0.487} & {0.511} & \textbf{0.469} & {0.498} & {0.489} \\
		\cline{4-20}
		& & & 1000 & {0.481} & \textbf{0.459} & {0.494} & {0.477} & {0.490} & \textbf{0.462} & {0.495} & {0.483} & {0.494} & \textbf{0.464} & {0.496} & {0.487} & {0.500} & \textbf{0.466} & {0.498} & {0.489} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Ladybug} & \multirow{3}{*}{10.48} & \multirow{3}{*}{0.702} & 100 & {0.708} & \textbf{\color{red}0.693} & {0.872} & {0.707} & {0.711} & \textbf{\color{red}0.695} & {0.858} & {0.741} & {0.717} & \textbf{\color{red}0.694} & {1.075} & {0.869} & {0.718} & \textbf{\color{red}0.694} & {1.023} & {0.885} \\
		\cline{4-20}
		& & & 500 & {\color{red}0.695} & \textbf{\color{red}0.690} & {0.846} & {\color{red}0.693} & {\color{red}0.698} & \textbf{\color{red}0.690} & {0.847} & {\color{red}0.694} & {\color{red}0.699} & \textbf{\color{red}0.690} & {0.854} & {\color{red}0.694} & {\color{red}0.700} & \textbf{\color{red}0.690} & {0.856} & {\color{red}0.694} \\
		\cline{4-20}
		& & & 1000 & {\color{red}0.693} & \textbf{\color{red}0.690} & {0.846} & {\color{red}0.693} & {\color{red}0.696} & \textbf{\color{red}0.690} & {0.847} & {\color{red}0.694} & {\color{red}0.696} & \textbf{\color{red}0.690} & {0.854} & {\color{red}0.694} & {\color{red}0.696} & \textbf{\color{red}0.690} & {0.856} & {\color{red}0.694} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Dubrovnik} & \multirow{3}{*}{3.765} & \multirow{3}{*}{0.423} & 100 & {0.476} & \textbf{0.440} & {2.013} & {0.495} & {0.750} & \textbf{0.558} & {2.046} & {0.509} & {0.860} & \textbf{0.641} & {2.072} & {0.511} & {0.865} & \textbf{0.648} & {2.073} & {0.518} \\
		\cline{4-20}
		& & & 500 & {0.448} & \textbf{0.424} & {2.000} & {0.483} & {0.646} & \textbf{0.430} & {2.037} & {0.493} & {0.742} & \textbf{0.445} & {2.066} & {0.491} & {0.747} & \textbf{0.462} & {2.067} & {0.501} \\
		\cline{4-20}
		& & & 1000 & {0.442} & \textbf{\color{red}0.423} & {2.000} & {0.483} & {0.591} & \textbf{\color{red}0.423} & {2.037} & {0.493} & {0.679} & \textbf{0.427} & {2.066} & {0.491} & {0.685} & \textbf{0.445} & {2.067} & {0.501} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Venice} & \multirow{3}{*}{26.33} & \multirow{3}{*}{0.467} & 100 & {0.518} & \textbf{0.479} & {0.516} & {0.662} & {0.523} & \textbf{0.480} & {0.517} & {0.761} & {0.535} & \textbf{0.491} & {0.519} & {1.503} & {0.545} & \textbf{0.495} & {0.520} & {3.684} \\
		\cline{4-20}
		& & & 500 & {0.490} & \textbf{\color{red}0.466} & {0.515} & {0.548} & {0.494} & \textbf{\color{red}0.466} & {0.516} & {0.589} & {0.506} & \textbf{0.472} & {0.517} & {0.838} & {0.513} & \textbf{0.475} & {0.518} & {1.094} \\
		\cline{4-20}
		& & & 1000 & {0.482} & \textbf{\color{red}0.465} & {0.515} & {0.547} & {0.484} & \textbf{\color{red}0.465} & {0.516} & {0.569} & {0.495} & \textbf{\color{red}0.467} & {0.517} & {0.833} & {0.500} & \textbf{0.474} & {0.518} & {1.094} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Final} & \multirow{3}{*}{12.57} & \multirow{3}{*}{0.848} & 100 & {0.975} & \textbf{0.860} & {2.078} & {1.017} & {1.101} & \textbf{0.912} & {2.138} & {1.396} & {1.117} & \textbf{0.889} & {2.173} & {4.643} & {1.356} & \textbf{0.951} & {2.288} & {1.111} \\
		\cline{4-20}
		& & & 500 & {0.894} & \textbf{\color{red}0.829} & {2.030} & {0.945} & {0.971} & \textbf{\color{red}0.830} & {2.086} & {1.396} & {0.954} & \textbf{\color{red}0.836} & {2.121} & {1.018} & {1.076} & \textbf{0.849} & {2.227} & {1.012} \\
		\cline{4-20}
		& & & 1000 & {0.870} & \textbf{\color{red}0.826} & {2.030} & {0.945} & {0.926} & \textbf{\color{red}0.827} & {2.086} & {0.991} & {0.907} & \textbf{\color{red}0.830} & {2.120} & {1.018} & {0.989} & \textbf{\color{red}0.842} & {2.227} & {1.003} \\
		\hline
		\hline
	
		
		\multicolumn{20}{|c|}{1DSfM \cite{wilson2014robust}}\\
		\hline
		\multirow{3}{*}{\scriptsize\sf Alamo} & \multirow{3}{*}{3.616} & \multirow{3}{*}{1.157} & 100 & {1.545} & \textbf{1.299} & {1.559} & {1.475} & {1.630} & \textbf{1.318} & {1.576} & {1.570} & {1.724} & \textbf{1.253} & {1.603} & {2.840} & {1.917} & \textbf{1.340} & {1.610} & {1.729} \\
		\cline{4-20}
		& & & 500 & {1.341} & \textbf{1.212} & {1.541} & {1.370} & {1.370} & \textbf{1.220} & {1.559} & {1.456} & {1.394} & \textbf{\color{red}1.152} & {1.575} & {1.534} & {1.443} & \textbf{1.227} & {1.594} & {1.621} \\
		\cline{4-20}
		& & & 1000 & {1.311} & \textbf{1.194} & {1.541} & {1.370} & {1.333} & \textbf{1.200} & {1.559} & {1.456} & {1.345} & \textbf{\color{red}1.141} & {1.575} & {1.534} & {1.362} & \textbf{1.206} & {1.594} & {1.621} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Ellis Island} & \multirow{3}{*}{11.98} & \multirow{3}{*}{5.022} & 100 & {6.530} & \textbf{5.580} & {8.124} & {8.798} & {6.997} & \textbf{5.835} & {8.562} & {11.98} & {7.388} & \textbf{5.920} & {8.597} & {11.98} & {7.583} & \textbf{5.969} & {9.901} & {11.98} \\
		\cline{4-20}
		& & & 500 & {5.878} & \textbf{5.100} & {6.866} & {5.257} & {6.169} & \textbf{5.369} & {6.937} & {5.325} & {6.411} & \textbf{5.307} & {7.012} & {5.432} & {6.502} & \textbf{5.181} & {7.066} & {5.516} \\
		\cline{4-20}
		& & & 1000 & {5.698} & \textbf{\color{red}5.001} & {6.866} & {5.257} & {5.929} & \textbf{5.260} & {6.937} & {5.325} & {6.094} & \textbf{5.190} & {7.012} & {5.432} & {6.157} & \textbf{5.116} & {7.066} & {5.516} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Gen. Markt} & \multirow{3}{*}{8.181} & \multirow{3}{*}{4.026} & 100 & {4.698} & \textbf{4.133} & {5.110} & {6.521} & {4.928} & \textbf{4.178} & {4.907} & {5.860} & {5.412} & \textbf{4.311} & {5.699} & {7.950} & {5.669} & \textbf{4.412} & {5.038} & {6.708} \\
		\cline{4-20}
		& & & 500 & {4.268} & \textbf{\color{red}4.010} & {4.848} & {4.361} & {4.366} & \textbf{\color{red}4.019} & {4.870} & {4.450} & {4.593} & \textbf{4.027} & {4.914} & {4.560} & {4.795} & \textbf{4.081} & {4.949} & {4.726} \\
		\cline{4-20}
		& & & 1000 & {4.138} & \textbf{\color{red}3.998} & {4.848} & {4.361} & {4.223} & \textbf{\color{red}4.009} & {4.870} & {4.450} & {4.362} & \textbf{\color{red}4.011} & {4.914} & {4.560} & {4.507} & \textbf{4.045} & {4.949} & {4.726} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf M. Metro.} & \multirow{3}{*}{4.599} & \multirow{3}{*}{2.379} & 100 & {2.921} & \textbf{2.553} & {3.746} & {3.424} & {2.926} & \textbf{2.524} & {2.841} & {3.111} & {3.123} & \textbf{2.570} & {4.183} & {4.599} & {3.227} & \textbf{2.613} & {3.027} & {4.599} \\
		\cline{4-20}
		& & & 500 & {2.609} & \textbf{2.395} & {2.793} & {2.558} & {2.603} & \textbf{2.428} & {2.795} & {2.638} & {2.703} & \textbf{2.413} & {2.810} & {2.729} & {2.772} & \textbf{2.438} & {2.821} & {2.830} \\
		\cline{4-20}
		& & & 1000 & {2.552} & \textbf{\color{red}2.368} & {2.793} & {2.558} & {2.531} & \textbf{2.401} & {2.795} & {2.637} & {2.601} & \textbf{2.387} & {2.810} & {2.729} & {2.653} & \textbf{2.408} & {2.821} & {2.830} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf M. N. Dame} & \multirow{3}{*}{7.335} & \multirow{3}{*}{3.706} & 100 & {4.177} & \textbf{3.730} & {4.433} & {3.975} & {4.368} & \textbf{3.764} & {4.469} & {4.166} & {4.507} & \textbf{3.774} & {4.490} & {4.352} & {4.608} & \textbf{3.781} & {4.515} & {4.529} \\
		\cline{4-20}
		& & & 500 & {3.817} & \textbf{\color{red}3.701} & {4.411} & {3.919} & {3.887} & \textbf{3.709} & {4.447} & {4.084} & {3.932} & \textbf{3.708} & {4.469} & {4.244} & {3.963} & \textbf{3.710} & {4.493} & {4.439} \\
		\cline{4-20}
		& & & 1000 & {3.752} & \textbf{\color{red}3.697} & {4.411} & {3.919} & {3.797} & \textbf{\color{red}3.702} & {4.447} & {4.084} & {3.817} & \textbf{\color{red}3.701} & {4.469} & {4.244} & {3.831} & \textbf{\color{red}3.704} & {4.493} & {4.439} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf N. Dame} & \multirow{3}{*}{9.442} & \multirow{3}{*}{3.312} & 100 & {4.118} & \textbf{3.487} & {3.769} & {3.671} & {4.174} & \textbf{3.560} & {3.801} & {5.574} & {4.358} & \textbf{3.548} & {4.116} & {4.443} & {4.399} & \textbf{3.571} & {4.136} & {4.895} \\
		\cline{4-20}
		& & & 500 & {3.652} & \textbf{3.345} & {3.742} & {3.622} & {3.685} & \textbf{3.329} & {3.758} & {3.694} & {3.753} & \textbf{3.348} & {3.784} & {3.771} & {3.772} & \textbf{3.348} & {3.793} & {3.861} \\
		\cline{4-20}
		& & & 1000 & {3.532} & \textbf{3.333} & {3.742} & {3.622} & {3.577} & \textbf{\color{red}3.309} & {3.758} & {3.693} & {3.606} & \textbf{3.333} & {3.784} & {3.771} & {3.626} & \textbf{3.333} & {3.793} & {3.861} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf NYC Library} & \multirow{3}{*}{5.140} & \multirow{3}{*}{1.889} & 100 & {2.371} & \textbf{1.937} & {2.535} & {2.140} & {2.514} & \textbf{1.949} & {2.844} & {2.173} & {2.648} & \textbf{1.988} & {2.595} & {2.500} & {2.853} & \textbf{2.046} & {2.566} & {3.011} \\
		\cline{4-20}
		& & & 500 & {2.018} & \textbf{\color{red}1.857} & {2.402} & {2.037} & {2.052} & \textbf{\color{red}1.860} & {2.425} & {2.069} & {2.113} & \textbf{\color{red}1.876} & {2.442} & {2.132} & {2.215} & \textbf{1.896} & {2.469} & {2.237} \\
		\cline{4-20}
		& & & 1000 & {1.962} & \textbf{\color{red}1.847} & {2.402} & {2.037} & {1.978} & \textbf{\color{red}1.854} & {2.425} & {2.069} & {2.021} & \textbf{\color{red}1.866} & {2.442} & {2.132} & {2.097} & \textbf{\color{red}1.881} & {2.469} & {2.237} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf P. del Popolo} & \multirow{3}{*}{6.552} & \multirow{3}{*}{2.371} & 100 & {3.383} & \textbf{2.552} & {3.034} & {2.625} & {3.631} & \textbf{2.624} & {3.326} & {5.340} & {3.812} & \textbf{2.640} & {3.404} & {3.150} & {3.946} & \textbf{2.684} & {3.410} & {3.276} \\
		\cline{4-20}
		& & & 500 & {2.856} & \textbf{2.407} & {3.009} & {2.574} & {2.943} & \textbf{\color{red}2.368} & {3.038} & {2.695} & {3.019} & \textbf{2.380} & {3.055} & {2.848} & {3.105} & \textbf{2.395} & {3.080} & {3.079} \\
		\cline{4-20}
		& & & 1000 & {2.692} & \textbf{2.397} & {3.009} & {2.574} & {2.784} & \textbf{\color{red}2.349} & {3.038} & {2.695} & {2.836} & \textbf{\color{red}2.355} & {3.055} & {2.848} & {2.897} & \textbf{\color{red}2.362} & {3.080} & {3.079} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Piccadily} & \multirow{3}{*}{11.26} & \multirow{3}{*}{4.392} & 100 & {5.736} & \textbf{4.762} & {9.146} & {11.26} & {5.688} & \textbf{4.727} & {6.729} & {9.290} & {6.290} & \textbf{4.988} & {10.29} & {11.26} & {6.592} & \textbf{5.187} & {10.18} & {11.26} \\
		\cline{4-20}
		& & & 500 & {5.088} & \textbf{\color{red}4.376} & {6.075} & {4.516} & {5.073} & \textbf{\color{red}4.326} & {6.067} & {4.542} & {5.445} & \textbf{4.403} & {6.162} & {4.682} & {5.665} & \textbf{4.485} & {6.214} & {4.720} \\
		\cline{4-20}
		& & & 1000 & {4.902} & \textbf{\color{red}4.299} & {6.075} & {4.515} & {4.874} & \textbf{\color{red}4.256} & {6.067} & {4.542} & {5.163} & \textbf{\color{red}4.339} & {6.150} & {4.682} & {5.351} & \textbf{\color{red}4.379} & {6.214} & {4.720} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf R. Forum} & \multirow{3}{*}{6.407} & \multirow{3}{*}{1.177} & 100 & {1.622} & \textbf{1.316} & {2.218} & {1.923} & {1.962} & \textbf{1.443} & {2.244} & {2.908} & {2.380} & \textbf{1.513} & {2.280} & {2.880} & {2.488} & \textbf{1.545} & {2.350} & {3.013} \\
		\cline{4-20}
		& & & 500 & {1.417} & \textbf{1.179} & {2.193} & {1.500} & {1.588} & \textbf{1.245} & {2.220} & {1.593} & {1.734} & \textbf{1.272} & {2.253} & {1.678} & {1.787} & \textbf{1.272} & {2.268} & {1.773} \\
		\cline{4-20}
		& & & 1000 & {1.366} & \textbf{\color{red}1.159} & {2.193} & {1.500} & {1.481} & \textbf{1.195} & {2.220} & {1.593} & {1.594} & \textbf{1.214} & {2.253} & {1.678} & {1.618} & \textbf{1.241} & {2.268} & {1.773} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf T. of London} & \multirow{3}{*}{4.399} & \multirow{3}{*}{0.669} & 100 & {0.994} & \textbf{0.756} & {1.193} & {1.056} & {1.050} & \textbf{0.742} & {1.211} & {0.960} & {1.315} & \textbf{0.787} & {1.233} & {0.891} & {1.487} & \textbf{0.810} & {1.262} & {0.992} \\
		\cline{4-20}
		& & & 500 & {0.814} & \textbf{0.685} & {1.174} & {0.775} & {0.820} & \textbf{\color{red}0.667} & {1.190} & {0.801} & {0.920} & \textbf{0.685} & {1.213} & {0.838} & {0.965} & \textbf{0.704} & {1.240} & {0.891} \\
		\cline{4-20}
		& & & 1000 & {0.777} & \textbf{\color{red}0.665} & {1.174} & {0.775} & {0.770} & \textbf{\color{red}0.659} & {1.190} & {0.801} & {0.831} & \textbf{0.673} & {1.213} & {0.838} & {0.856} & \textbf{0.685} & {1.240} & {0.891} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Trafalgar} & \multirow{3}{*}{10.77} & \multirow{3}{*}{3.739} & 100 & {4.928} & \textbf{4.012} & {7.167} & {10.76} & {5.538} & \textbf{4.123} & {6.702} & {10.77} & {6.033} & \textbf{4.332} & {8.494} & {10.77} & {6.462} & \textbf{4.518} & {9.206} & {10.77} \\
		\cline{4-20}
		& & & 500 & {4.276} & \textbf{\color{red}3.680} & {5.239} & {3.880} & {4.522} & \textbf{\color{red}3.689} & {5.144} & {3.982} & {4.853} & \textbf{\color{red}3.726} & {5.661} & {4.084} & {5.160} & \textbf{3.782} & {5.389} & {4.234} \\
		\cline{4-20}
		& & & 1000 & {4.096} & \textbf{\color{red}3.632} & {5.239} & {3.880} & {4.231} & \textbf{\color{red}3.633} & {5.144} & {3.982} & {4.485} & \textbf{\color{red}3.652} & {5.551} & {4.083} & {4.744} & \textbf{\color{red}3.688} & {5.286} & {4.234} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf U. Square} & \multirow{3}{*}{10.57} & \multirow{3}{*}{3.978} & 100 & {5.074} & \textbf{4.382} & {9.273} & {6.428} & {5.602} & \textbf{4.461} & {8.395} & {10.57} & {5.914} & \textbf{4.707} & {8.959} & {10.57} & {6.227} & \textbf{4.876} & {10.57} & {10.57} \\
		\cline{4-20}
		& & & 500 & {4.629} & \textbf{\color{red}3.972} & {5.387} & {4.195} & {4.834} & \textbf{4.005} & {5.452} & {4.217} & {5.103} & \textbf{4.098} & {5.509} & {4.305} & {5.350} & \textbf{4.158} & {5.563} & {4.395} \\
		\cline{4-20}
		& & & 1000 & {4.491} & \textbf{\color{red}3.914} & {5.387} & {4.195} & {4.597} & \textbf{\color{red}3.931} & {5.452} & {4.217} & {4.851} & \textbf{3.998} & {5.509} & {4.305} & {5.033} & \textbf{4.024} & {5.563} & {4.395} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf V. Cathedral} & \multirow{3}{*}{9.506} & \multirow{3}{*}{1.96} & 100 & {2.830} & \textbf{1.994} & {3.245} & {2.964} & {2.917} & \textbf{1.982} & {3.264} & {5.063} & {3.212} & \textbf{2.102} & {3.327} & {4.657} & {3.699} & \textbf{2.191} & {3.388} & {2.941} \\
		\cline{4-20}
		& & & 500 & {2.201} & \textbf{\color{red}1.795} & {3.139} & {2.148} & {2.199} & \textbf{\color{red}1.796} & {3.150} & {2.202} & {2.373} & \textbf{\color{red}1.842} & {3.212} & {2.297} & {2.569} & \textbf{\color{red}1.868} & {3.289} & {2.427} \\
		\cline{4-20}
		& & & 1000 & {2.049} & \textbf{\color{red}1.746} & {3.139} & {2.148} & {2.042} & \textbf{\color{red}1.757} & {3.150} & {2.202} & {2.184} & \textbf{\color{red}1.813} & {3.212} & {2.297} & {2.267} & \textbf{\color{red}1.832} & {3.289} & {2.427} \\
		\hline
		\hline
		\multirow{3}{*}{\scriptsize\sf Y. Minster} & \multirow{3}{*}{8.929} & \multirow{3}{*}{1.987} & 100 & {2.804} & \textbf{2.061} & {3.304} & {2.432} & {3.246} & \textbf{2.212} & {3.380} & {2.457} & {3.570} & \textbf{2.250} & {3.437} & {3.061} & {3.710} & \textbf{2.335} & {6.113} & {7.743} \\
		\cline{4-20}
		& & & 500 & {2.361} & \textbf{\color{red}1.934} & {3.254} & {2.241} & {2.408} & \textbf{\color{red}1.986} & {3.331} & {2.296} & {2.561} & \textbf{\color{red}1.965} & {3.388} & {2.413} & {2.655} & \textbf{\color{red}1.952} & {3.431} & {2.573} \\
		\cline{4-20}
		& & & 1000 & {2.265} & \textbf{\color{red}1.923} & {3.254} & {2.241} & {2.245} & \textbf{\color{red}1.953} & {3.331} & {2.296} & {2.368} & \textbf{\color{red}1.941} & {3.388} & {2.413} & {2.404} & \textbf{\color{red}1.928} & {3.431} & {2.573} \\
		\hline
	\end{tabular}
	\vspace{-0.75em}
\end{table*}	


==> table/table_datasets.tex <==
\begin{table}[t]
	\centering
	\setlength{\tabcolsep}{0.3em}
	\caption{Largest Bundle adjustment datasets of more than 700 cameras in BAL \cite{agarwal2010bundle} and 1DSfM \cite{wilson2014robust}.}\label{table::dataset}
	\begin{tabular}{|P{0.09\textwidth}|P{0.075\textwidth}|P{0.08\textwidth}|P{0.1\textwidth}|}
		\hline			
		Dataset & \# Cameras & \# Points &\# Observations  \\
		\hline
		\multicolumn{4}{|c|}{BAL \cite{agarwal2010bundle}}\\
		\hline
		%{\scriptsize\sf Trafalgar} & 257 & 65132 & 225911  \\
		\hline
 		{\scriptsize\sf Ladybug} & 1723 & 156502 & 678718  \\
		\hline
		%{\scriptsize\sf Dubrovnik} & 356 & 226730 & 1255268  \\
		% \hline
		{\scriptsize\sf Venice} & 1778 & 993923 & 5001946  \\
		\hline
		{\scriptsize\sf Final} & 13682 & 4456117 & 28987644 \\
		\hline
		\multicolumn{4}{|c|}{1DSfM \cite{wilson2014robust}}\\
		\hline
		%{\scriptsize\sf Alamo} & 571 & 151085 & 891301  \\
		% \hline
		% {\scriptsize\sf Ellis Island} & 234 & 29164 & 130903  \\
		% \hline
		{\scriptsize\sf Gen. Markt} & 706 & 93672 & 364029  \\
		\hline
		% {\scriptsize\sf M. Metropolis} & 346 & 55679 & 255987  \\
		% \hline
		% {\scriptsize\sf M. N. Dame} & 459 & 158005 & 860116 \\
		% \hline
		% {\scriptsize\sf N. Dame} & 547 & 273590 & 1534747 \\
		% \hline
		% {\scriptsize\sf NYC Library} & 338 & 74249 & 303955  \\
		% \hline
		% {\scriptsize\sf P. del Popolo} & 335 & 37609 & 195016  \\
		% \hline
		{\scriptsize\sf Piccadilly} & 2289 & 209504 & 999878  \\
		\hline
		{\scriptsize\sf R. Forum} & 1063 & 265047 &  1292756  \\
		\hline
		% {\scriptsize\sf T. of London} & 483 & 151328 & 797022  \\
		% \hline
		{\scriptsize\sf Trafalgar} & 5032 & 388956 & 1826071  \\
		\hline
		{\scriptsize\sf U. Square} & 796 & 46066 & 230811  \\
		\hline
		{\scriptsize\sf V. Cathedral} & 836 & 265553 & 1333280 \\
		\hline
		% {\scriptsize\sf Y. Minster} & 422 & 152591 & 701989  \\
		% \hline
	\end{tabular}
    \vspace{-0.5em}
\end{table}
